Does Microservices Adoption Impact the Development Velocity? A Cohort Study. A Registered Report

[Context] Microservices enable the decomposition of applications into small and independent services connected together. The independence between services could positively affect the development velocity of a project, which is considered an important metric measuring the time taken to implement features and fix bugs. However, no studies have investigated the connection between microservices and development velocity. [Objective and Method] The goal of this study plan is to investigate the effect microservices have on development velocity. The study compares GitHub projects adopting microservices from the beginning and similar projects using monolithic architectures. We designed this study using a cohort study method, to enable obtaining a high level of evidence. [Results] The result of this work enables the confirmation of the effective improvement of the development velocity of microservices. Moreover, this study will contribute to the body of knowledge of empirical methods being among the first works adopting the cohort study methodology.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> Section/Execution.tex <==
\section{Execution Plan}
\label{sec:Execution}

% \todo[inline]{Discuss about how well the study methodology suits doing SE/MSR studies}

==> Section/RelatedWork.tex <==
\section{Related work}
\label{sec:related_work}
% \subsection{Empirical method}
% \todo[inline]{might not be needed depending on the intro \\
% Davide thought this is not needed}

% \subsection{Empirical studies about Docker}
% \todo[inline]{@Davide}
% Traditional related work



==> Section/Results.tex <==
\section{Results}

\subsection{Participants}
%Report numbers of individuals at each stage of study—eg numbers potentially eligible, examined for eligibility, confirmed eligible, included in the study, completing follow-up, and analysed

\subsection{Descriptive data}
%- Give characteristics of study participants (eg demographic, clinical, social) and information on exposures and potential confounders
%- Number of participants with missing data
%- summarise follow-up time

\subsection{Outcome data}
%Report numbers of outcome events or summary measures over tim

\subsection{Main results}
%Give unadjusted estimates and, if applicable, confounder-adjusted estimates and their precision (eg, 95\% confidence interval). Make clear which confounders were adjusted for and why they were included

\subsection{Other analyses}
%Report other analyses done — eg analyses of subgroups and interactions, and sensitivity analyses

==> Section/RiskManagement.tex <==
\section{Risk management} \label{sec:RiskManagement}
This section addresses the possible risks that could happen during the study, as well as the strategy designed to mitigate the effects of the same risks.

\textbf{Data shortage.} Given the large amount of projects existing in GitHub we expect to have enough data that matches the minimum sample size determined in Section 4.7. However, the exclusion criteria we set for this study might lead to a sharp reduction of analyzable projects. To mitigate this,  we would consider collecting projects from additional data sources, such as GitLab, as well as Jira or Bugzilla for issue tracking.
%\todo[inline]{Mikel [24/5]: This is covered in Internal validity, perhaps could fit in this section} \sv{Yes. Definitely, this fits better in this section.}

% \textbf{Failure in matching.}
% \textbf{Lack of significance in the statistical adjusment.}


==> meetingNote.tex <==
#### 30.11.2022 Meeting Note ####

Microservice developer affiliation

RQ1: 
Are developers commiting only on one ms in the same time? 

Is the one-microservice-per-developer pattern respected in oss microservices projects?

Dario:
	Dataset: 38 projects more than 2 developers and 2 commits
	Diagram: Project 46 commits but only 3 developers, 1 committer for 55 commits
	
	Call graphs: number of shared developers
	Larger line for ? 
	1) Chord diagram -> developers and MSs
	if 1 developer for 1 MS -> very messy
	
	1 develper 1 ms then move on to another one -> bad practice?
	in that case we can move the 2 ms into 1.
	For each project, 

Davide:
	Make identical, different colour for the lines, 
	if 2 developers -> commit everything
	1 developer for 1 color, the others another colour (chord diagram)
	
	2 problems: 1) visualise 1
	2) represent multiple projects, multiple MSs

	show some results meaningful
	Check the OSS project, if this practice is applied
	happened once or several times?

	We see RQs first and decide
	developer profiles?
	 
	Priority: show the collaboration with Developers then next step
	Only RQ1 immediately, write the results, then go forward.
	
	Statistics? -> 
	Which type of data analysis? 40 projects, each project has different MSs and different developers, age of the projects, What info we need to answer the RQ? 
Each project: AVG number of Ms each Developers work on, Max, Min, AVG MS per developers (= MAX-MS-X-DEVELOPERS;MIN-MS-X-DEVELOPERS;AVG-MS-X-DEVELOPERS;PERCENTAGE-OF-DEVELOPERS-COMMTTING-ON-ONLY-1-MS) 
Count number of developers working on 1 MS. count percentage of 1 developers on 1 MS (properly developing) -> answering RQ
Kmeans. Project number of developers, with threashold, then cluster the projects. Developer numbers, ages, total number of commits …. 
Bloxplot. Describe the clusters. 
Number of developers developing only 1 MS. -> Percentage by the total number 
Sort by a reasonable/meaningful way

Perfect to have a boxplot flat 1.

Andrea:
	lines for MS should be something in common
	-> diagram showing problems
	-> in certain context, team work that way, shown in the diagram.
	-> collaboration in 1 MS with another diagram
	show the collaboration? 
	show the trends?
	-> From diagrams to detect patterns
	Extend to : How well is 1 developer pattern be respected … 
	the percentage of the clusters in details later finding insights.

Vale:
	1 developer to 1 MS: coincidence or good practice
	T-test?
	This to the 2nd iteration

MEETING 5/12/2022
- Davide rule: count the number of "single developer commit changes".

